MultiCast: Zero-Shot Multivariate Time Series Forecasting Using LLMs

Predicting future values in multivariate time series is vital across various domains. This work explores the use of large language models (LLMs) for this task. However, LLMs typically handle one-dimensional data. We introduce MultiCast, a zero-shot LLM-based approach for multivariate time series forecasting. It allows LLMs to receive multivariate time series as input, through three novel token multiplexing solutions that effectively reduce dimensionality while preserving key repetitive patterns. Additionally, a quantization scheme helps LLMs to better learn these patterns, while significantly reducing token use for practical applications. We showcase the performance of our approach in terms of RMSE and execution time against state-of-the-art approaches on three real-world datasets.

==> Preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

% \subsection{SAX Representation of Time Series}
% \label{subsec:sax}

% The {\em Symbolic Aggregate approXimation (SAX)} is a multi-resolution representation of a time series introduced in \cite{shieh2008kdd}. It can be derived from its {\em Piecewise Aggregate Approximation} (PAA) \cite{keogh2001paa,faloutsos2000vldb} by quantizing the PAA segments on the $v$-axis. As exemplified in Figure~\ref{fig:isax_representation}, a time series $T_2$ is transformed into a PAA representation of $w$=3 words with real-valued coefficients (the horizontal red bars). To obtain a $SAX$ representation for a time series, these coefficients are discretized along the value axis using {\em breakpoints} (shown with dashed lines) assuming a $\mathcal{N}(0,1)$ Gaussian distribution that enables generation of equiprobable symbols for a given cardinality ($b=4$ symbols are used in this example). Although bitwise representations were used for these symbols in the original paper, other encoding types are also possible. Two such popular alternatives are using alphabetical characters or digits for each symbol.

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.55\columnwidth]{Figures/sax2.pdf}
% 	\caption{SAX representation of a time series.}
% 	\label{fig:isax_representation}
% \end{figure}



==> References_BAK.tex <==
@inproceedings{shieh2008kdd,
  author    = {Jin Shieh and Eamonn J. Keogh},
  title     = {\emph{i}{SAX}: indexing and mining terabyte sized time series},
  booktitle = {{SIGKDD}},
  pages     = {623--631},
  year      = {2008}
}

@inproceedings{faloutsos2000vldb,
  author    = {Byoung{-}Kee Yi and
               Christos Faloutsos},
  title     = {Fast Time Sequence Indexing for Arbitrary {Lp} Norms},
  @booktitle = {{VLDB} 2000, Proceedings of 26th International Conference on Very
               Large Data Bases, September 10-14, 2000, Cairo, Egypt},
  booktitle = {{VLDB}},
  pages     = {385--394},
  year      = {2000}
}

@article{keogh2001paa,
  author    = {Eamonn J. Keogh and
               Kaushik Chakrabarti and
               Michael J. Pazzani and
               Sharad Mehrotra},
  title     = {Dimensionality Reduction for Fast Similarity Search in Large Time
               Series Databases},
  journal   = {Knowl. Inf. Syst.},
  volume    = {3},
  number    = {3},
  pages     = {263--286},
  year      = {2001}
}

@article{gruver2023large,
  title={Large language models are zero-shot time series forecasters},
  author={Gruver, Nate and Finzi, Marc and Qiu, Shikai and Wilson, Andrew Gordon},
  journal={arXiv preprint arXiv:2310.07820},
  year={2023}
}

@book{box2015time,
  title={Time series analysis: forecasting and control},
  author={Box, George EP and Jenkins, Gwilym M and Reinsel, Gregory C and Ljung, Greta M},
  year={2015},
  publisher={John Wiley \& Sons}
}

@article{lstm97,
    author = {Hochreiter, Sepp and Schmidhuber, Jürgen},
    year = {1997},
    month = {12},
    pages = {1735-80},
    title = {Long Short-term Memory},
    volume = {9},
    journal = {Neural computation},
    doi = {10.1162/neco.1997.9.8.1735}
}

@inproceedings{alhirmizy2019multivariate,
  title={Multivariate time series forecasting with LSTM for Madrid, Spain pollution},
  author={Alhirmizy, Shaheen and Qader, Banaz},
  booktitle={2019 international conference on computing and information science and technology and their applications (ICCISTA)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}

@article{ju2021multivariate,
  title={Multivariate time series data prediction based on att-lstm network},
  author={Ju, Jie and Liu, Fang-Ai},
  journal={Applied sciences},
  volume={11},
  number={20},
  pages={9373},
  year={2021},
  publisher={MDPI}
}


@ARTICLE{9461796,
  author={Liu, Zhenyu and Zhu, Zhengtong and Gao, Jing and Xu, Cheng},
  journal={IEEE Access}, 
  title={Forecast Methods for Time Series Data: A Survey}, 
  year={2021},
  volume={9},
  number={},
  pages={91896-91912},
  doi={10.1109/ACCESS.2021.3091162}
}

@article{DEGOOIJER2006443,
title = {25 years of time series forecasting},
journal = {International Journal of Forecasting},
volume = {22},
number = {3},
pages = {443-473},
year = {2006},
issn = {0169-2070},
doi = {https://doi.org/10.1016/j.ijforecast.2006.01.001},
author = {Jan G. {De Gooijer} and Rob J. Hyndman}
}

@InProceedings{10.1007/11579427_51,
author="Kuvulmaz, Janset
and Usanmaz, Serkan
and Engin, Seref Naci",
editor="Gelbukh, Alexander
and de Albornoz, {\'A}lvaro
and Terashima-Mar{\'i}n, Hugo",
title="Time-Series Forecasting by Means of Linear and Nonlinear Models",
booktitle="MICAI 2005: Advances in Artificial Intelligence",
year="2005",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="504--513"
}

@article{doi:10.1080/0740817X.2014.999180,
author = {Changqing Cheng and Akkarapol Sa-Ngasoongsong and Omer Beyca and Trung Le and Hui Yang and Zhenyu Kong and Satish Bukkapatnam},
title = {Time series forecasting for nonlinear and non-stationary processes: a review and comparative study},
journal = {IIE Transactions},
volume = {47},
number = {10},
pages = {1053-1071},
year = {2015},
publisher = {Taylor & Francis},
doi = {10.1080/0740817X.2014.999180}
}

@article{10.1145/3533382,
author = {Benidis, Konstantinos and Rangapuram, Syama Sundar and Flunkert, Valentin and Wang, Yuyang and Maddix, Danielle and Turkmen, Caner and Gasthaus, Jan and Bohlke-Schneider, Michael and Salinas, David and Stella, Lorenzo and Aubet, Fran\c{c}ois-Xavier and Callot, Laurent and Januschowski, Tim},
title = {Deep Learning for Time Series Forecasting: Tutorial and Literature Survey},
year = {2022},
issue_date = {June 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {55},
number = {6},
issn = {0360-0300},
url = {https://doi.org/10.1145/3533382},
doi = {10.1145/3533382},
journal = {ACM Comput. Surv.},
month = {dec},
articleno = {121},
numpages = {36},
}

@article{doi:10.1089/big.2020.0159,
author = {Torres, Jos\'{e} F. and Hadjout, Dalil and Sebaa, Abderrazak and Mart\'{\i}nez-\'{A}lvarez, Francisco and Troncoso, Alicia},
title = {Deep Learning for Time Series Forecasting: A Survey},
journal = {Big Data},
volume = {9},
number = {1},
pages = {3-21},
year = {2021},
doi = {10.1089/big.2020.0159}
}

@article{DU2020269,
title = {Multivariate time series forecasting via attention-based encoder–decoder framework},
journal = {Neurocomputing},
volume = {388},
pages = {269-279},
year = {2020},
issn = {0925-2312},
doi = {https://doi.org/10.1016/j.neucom.2019.12.118},
author = {Shengdong Du and Tianrui Li and Yan Yang and Shi-Jinn Horng}
}

@misc{jiang2022transferability,
      title={Transferability in Deep Learning: A Survey}, 
      author={Junguang Jiang and Yang Shu and Jianmin Wang and Mingsheng Long},
      year={2022},
      eprint={2201.05867},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@Inbook{Mahmoud2021,
author="Mahmoud, Amal
and Mohammed, Ammar",
editor="Hassanien, Aboul Ella and Darwish, Ashraf",
title="A Survey on Deep Learning for Time-Series Forecasting",
bookTitle="Machine Learning and Big Data Analytics Paradigms: Analysis, Applications and Challenges",
year="2021",
publisher="Springer International Publishing",
pages="365--392",
doi="10.1007/978-3-030-59338-4_19"
}

@article{Zeng_Chen_Zhang_Xu_2023,
title={Are Transformers Effective for Time Series Forecasting?},
volume={37}, 
DOI={10.1609/aaai.v37i9.26317}, 
number={9},
journal={Proceedings of the AAAI Conference on Artificial Intelligence},
author={Zeng, Ailing and Chen, Muxi and Zhang, Lei and Xu, Qiang},
year={2023},
month={Jun.},
pages={11121-11128}
}


@inproceedings{Radford2019LanguageMA,
  title={Language Models are Unsupervised Multitask Learners},
  author={Alec Radford and Jeff Wu and Rewon Child and David Luan and Dario Amodei and Ilya Sutskever},
  year={2019},
  journal={OpenAI}
}




@inproceedings{DBLP:conf/naacl/DevlinCLT19,
  author       = {Jacob Devlin and
                  Ming{-}Wei Chang and
                  Kenton Lee and
                  Kristina Toutanova},
  editor       = {Jill Burstein and
                  Christy Doran and
                  Thamar Solorio},
  title        = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
                  Understanding},
  booktitle    = {Proceedings of the 2019 Conference of the North American Chapter of
                  the Association for Computational Linguistics: Human Language Technologies,
                  {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
                  and Short Papers)},
  pages        = {4171--4186},
  publisher    = {Association for Computational Linguistics},
  year         = {2019},
  url          = {https://doi.org/10.18653/v1/n19-1423},
  doi          = {10.18653/V1/N19-1423},
  timestamp    = {Mon, 26 Sep 2022 12:21:55 +0200},
  biburl       = {https://dblp.org/rec/conf/naacl/DevlinCLT19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{10.5555/3455716.3455856,
author = {Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
title = {Exploring the limits of transfer learning with a unified text-to-text transformer},
year = {2020},
publisher = {JMLR.org},
volume = {21},
number = {1},
issn = {1532-4435},
journal = {J. Mach. Learn. Res.},
month = {jan},
numpages = {67},
}

@inproceedings{lewis-etal-2020-bart,
    title = "{BART}: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension",
    author = "Lewis, Mike  and
      Liu, Yinhan  and
      Goyal, Naman  and
      Ghazvininejad, Marjan  and
      Mohamed, Abdelrahman  and
      Levy, Omer  and
      Stoyanov, Veselin  and
      Zettlemoyer, Luke",
    editor = "Jurafsky, Dan  and
      Chai, Joyce  and
      Schluter, Natalie  and
      Tetreault, Joel",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    publisher = "Association for Computational Linguistics",
    doi = "10.18653/v1/2020.acl-main.703",
    pages = "7871--7880",
}

@misc{touvron2023llama,
      title={Llama 2: Open Foundation and Fine-Tuned Chat Models}, 
      author={Hugo Touvron and Louis Martin and Kevin Stone and Peter Albert and Amjad Almahairi and Yasmine Babaei and Nikolay Bashlykov and Soumya Batra and Prajjwal Bhargava and Shruti Bhosale and Dan Bikel and Lukas Blecher and Cristian Canton Ferrer and Moya Chen and Guillem Cucurull and David Esiobu and Jude Fernandes and Jeremy Fu and Wenyin Fu and Brian Fuller and Cynthia Gao and Vedanuj Goswami and Naman Goyal and Anthony Hartshorn and Saghar Hosseini and Rui Hou and Hakan Inan and Marcin Kardas and Viktor Kerkez and Madian Khabsa and Isabel Kloumann and Artem Korenev and Punit Singh Koura and Marie-Anne Lachaux and Thibaut Lavril and Jenya Lee and Diana Liskovich and Yinghai Lu and Yuning Mao and Xavier Martinet and Todor Mihaylov and Pushkar Mishra and Igor Molybog and Yixin Nie and Andrew Poulton and Jeremy Reizenstein and Rashi Rungta and Kalyan Saladi and Alan Schelten and Ruan Silva and Eric Michael Smith and Ranjan Subramanian and Xiaoqing Ellen Tan and Binh Tang and Ross Taylor and Adina Williams and Jian Xiang Kuan and Puxin Xu and Zheng Yan and Iliyan Zarov and Yuchen Zhang and Angela Fan and Melanie Kambadur and Sharan Narang and Aurelien Rodriguez and Robert Stojnic and Sergey Edunov and Thomas Scialom},
      year={2023},
      eprint={2307.09288},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{chowdhery2022palm,
      title={PaLM: Scaling Language Modeling with Pathways}, 
      author={Aakanksha Chowdhery and Sharan Narang and Jacob Devlin and Maarten Bosma and Gaurav Mishra and Adam Roberts and Paul Barham and Hyung Won Chung and Charles Sutton and Sebastian Gehrmann and Parker Schuh and Kensen Shi and Sasha Tsvyashchenko and Joshua Maynez and Abhishek Rao and Parker Barnes and Yi Tay and Noam Shazeer and Vinodkumar Prabhakaran and Emily Reif and Nan Du and Ben Hutchinson and Reiner Pope and James Bradbury and Jacob Austin and Michael Isard and Guy Gur-Ari and Pengcheng Yin and Toju Duke and Anselm Levskaya and Sanjay Ghemawat and Sunipa Dev and Henryk Michalewski and Xavier Garcia and Vedant Misra and Kevin Robinson and Liam Fedus and Denny Zhou and Daphne Ippolito and David Luan and Hyeontaek Lim and Barret Zoph and Alexander Spiridonov and Ryan Sepassi and David Dohan and Shivani Agrawal and Mark Omernick and Andrew M. Dai and Thanumalayan Sankaranarayana Pillai and Marie Pellat and Aitor Lewkowycz and Erica Moreira and Rewon Child and Oleksandr Polozov and Katherine Lee and Zongwei Zhou and Xuezhi Wang and Brennan Saeta and Mark Diaz and Orhan Firat and Michele Catasta and Jason Wei and Kathy Meier-Hellstern and Douglas Eck and Jeff Dean and Slav Petrov and Noah Fiedel},
      year={2022},
      eprint={2204.02311},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{Achiam2023GPT4TR,
  title={GPT-4 Technical Report},
  author={OpenAI Josh Achiam and Steven Adler and Sandhini Agarwal and Lama Ahmad and Ilge Akkaya and Florencia Leoni Aleman and Diogo Almeida and Janko Altenschmidt and Sam Altman and Shyamal Anadkat and Red Avila and Igor Babuschkin and Suchir Balaji and Valerie Balcom and Paul Baltescu and Haiming Bao and Mo Bavarian and Jeff Belgum and Irwan Bello and Jake Berdine and Gabriel Bernadett-Shapiro and Christopher Berner and Lenny Bogdonoff and Oleg Boiko and Madelaine Boyd and Anna-Luisa Brakman and Greg Brockman and Tim Brooks and Miles Brundage and Kevin Button and Trevor Cai and Rosie Campbell and Andrew Cann and Brittany Carey and Chelsea Carlson and Rory Carmichael and Brooke Chan and Che Chang and Fotis Chantzis and Derek Chen and Sully Chen and Ruby Chen and Jason Chen and Mark Chen and Benjamin Chess and Chester Cho and Casey Chu and Hyung Won Chung and Dave Cummings and Jeremiah Currier and Yunxing Dai and Cory Decareaux and Thomas Degry and Noah Deutsch and Damien Deville and Arka Dhar and David Dohan and Steve Dowling and Sheila Dunning and Adrien Ecoffet and Atty Eleti and Tyna Eloundou and David Farhi and Liam Fedus and Niko Felix and Sim'on Posada Fishman and Juston Forte and Isabella Fulford and Leo Gao and Elie Georges and Christian Gibson and Vik Goel and Tarun Gogineni and Gabriel Goh and Raphael Gontijo-Lopes and Jonathan Gordon and Morgan Grafstein and Scott Gray and Ryan Greene and Joshua Gross and Shixiang Shane Gu and Yufei Guo and Chris Hallacy and Jesse Han and Jeff Harris and Yuchen He and Mike Heaton and Johannes Heidecke and Chris Hesse and Alan Hickey and Wade Hickey and Peter Hoeschele and Brandon Houghton and Kenny Hsu and Shengli Hu and Xin Hu and Joost Huizinga and Shantanu Jain and Shawn Jain and Joanne Jang and Angela Jiang and Roger Jiang and Haozhun Jin and Denny Jin and Shino Jomoto and Billie Jonn and Heewoo Jun and Tomer Kaftan and Lukasz Kaiser and Ali Kamali and Ingmar Kanitscheider and Nitish Shirish Keskar and Tabarak Khan and Logan Kilpatrick and Jong Wook Kim and Christina Kim and Yongjik Kim and Hendrik Kirchner and Jamie Ryan Kiros and Matthew Knight and Daniel Kokotajlo and Lukasz Kondraciuk and Andrew Kondrich and Aris Konstantinidis and Kyle Kosic and Gretchen Krueger and Vishal Kuo and Michael Lampe and Ikai Lan and Teddy Lee and Jan Leike and Jade Leung and Daniel Levy and Chak Ming Li and Rachel Lim and Molly Lin and Stephanie Lin and Mateusz Litwin and Theresa Lopez and Ryan Lowe and Patricia Lue and Anna Adeola Makanju and Kim Malfacini and Sam Manning and Todor Markov and Yaniv Markovski and Bianca Martin and Katie Mayer and Andrew Mayne and Bob McGrew and Scott Mayer McKinney and Christine McLeavey and Paul McMillan and Jake McNeil and David Medina and Aalok Mehta and Jacob Menick and Luke Metz and Andrey Mishchenko and Pamela Mishkin and Vinnie Monaco and Evan Morikawa and Daniel P. Mossing and Tong Mu and Mira Murati and Oleg Murk and David M'ely and Ashvin Nair and Reiichiro Nakano and Rajeev Nayak and Arvind Neelakantan and Richard Ngo and Hyeonwoo Noh and Ouyang Long and Cullen O'Keefe and Jakub W. Pachocki and Alex Paino and Joe Palermo and Ashley Pantuliano and Giambattista Parascandolo and Joel Parish and Emy Parparita and Alexandre Passos and Mikhail Pavlov and Andrew Peng and Adam Perelman and Filipe de Avila Belbute Peres and Michael Petrov and Henrique Pond{\'e} de Oliveira Pinto and Michael Pokorny and Michelle Pokrass and Vitchyr H. Pong and Tolly Powell and Alethea Power and Boris Power and Elizabeth Proehl and Raul Puri and Alec Radford and Jack Rae and Aditya Ramesh and Cameron Raymond and Francis Real and Kendra Rimbach and Carl Ross and Bob Rotsted and Henri Roussez and Nick Ryder and Mario D. Saltarelli and Ted Sanders and Shibani Santurkar and Girish Sastry and Heather Schmidt and David Schnurr and John Schulman and Daniel Selsam and Kyla Sheppard and Toki Sherbakov and Jessica Shieh and Sarah Shoker and Pranav Shyam and Szymon Sidor and Eric Sigler and Maddie Simens and Jordan Sitkin and Katarina Slama and Ian Sohl and Benjamin D. Sokolowsky and Yang Song and Natalie Staudacher and Felipe Petroski Such and Natalie Summers and Ilya Sutskever and Jie Tang and Nikolas A. Tezak and Madeleine Thompson and Phil Tillet and Amin Tootoonchian and Elizabeth Tseng and Preston Tuggle and Nick Turley and Jerry Tworek and Juan Felipe Cer'on Uribe and Andrea Vallone and Arun Vijayvergiya and Chelsea Voss and Carroll Wainwright and Justin Jay Wang and Alvin Wang and Ben Wang and Jonathan Ward and Jason Wei and CJ Weinmann and Akila Welihinda and Peter Welinder and Jiayi Weng and Lilian Weng and Matt Wiethoff and Dave Willner and Clemens Winter and Samuel Wolrich and Hannah Wong and Lauren Workman and Sherwin Wu and Jeff Wu and Michael Wu and Kai Xiao and Tao Xu and Sarah Yoo and Kevin Yu and Qiming Yuan and Wojciech Zaremba and Rowan Zellers and Chong Zhang and Marvin Zhang and Shengjia Zhao and Tianhao Zheng and Juntang Zhuang and William Zhuk and Barret Zoph},
  year={2023},
  journal={OpenAI}
}


@misc{jiang2024empowering,
      title={Empowering Time Series Analysis with Large Language Models: A Survey}, 
      author={Yushan Jiang and Zijie Pan and Xikun Zhang and Sahil Garg and Anderson Schneider and Yuriy Nevmyvaka and Dongjin Song},
      year={2024},
      eprint={2402.03182},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{schmiedmayer2024llm,
  title={LLM on FHIR--Demystifying Health Records},
  author={Schmiedmayer, Paul and Rao, Adrit and Zagar, Philipp and Ravi, Vishnu and Zahedivash, Aydin and Fereydooni, Arash and Aalami, Oliver},
  journal={arXiv preprint arXiv:2402.01711},
  year={2024}
}

@article{nashwan2023harnessing,
  title={Harnessing the power of large language models (LLMs) for electronic health records (EHRs) optimization},
  author={Nashwan, Abdulqadir J and AbuJaber, Ahmad A and AbuJaber, Ahmad},
  journal={Cureus},
  volume={15},
  number={7},
  year={2023},
  publisher={Cureus}
}

@article{wornow2024zero,
  title={Zero-Shot Clinical Trial Patient Matching with LLMs},
  author={Wornow, Michael and Lozano, Alejandro and Dash, Dev and Jindal, Jenelle and Mahaffey, Kenneth W and Shah, Nigam H},
  journal={arXiv preprint arXiv:2402.05125},
  year={2024}
}

@misc{zhang2024large,
      title={Large Language Models for Time Series: A Survey}, 
      author={Xiyuan Zhang and Ranak Roy Chowdhury and Rajesh K. Gupta and Jingbo Shang},
      year={2024},
      eprint={2402.01801},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{li2023large,
  title={Large language models in finance: A survey},
  author={Li, Yinheng and Wang, Shaofei and Ding, Han and Chen, Hang},
  booktitle={Proceedings of the Fourth ACM International Conference on AI in Finance},
  pages={374--382},
  year={2023}
}

@article{yang2023fingpt,
  title={FinGPT: Open-Source Financial Large Language Models},
  author={Yang, Hongyang and Liu, Xiao-Yang and Wang, Christina Dan},
  journal={arXiv preprint arXiv:2306.06031},
  year={2023}
}

@article{hadi2023survey,
  title={A survey on large language models: Applications, challenges, limitations, and practical usage},
  author={Hadi, Muhammad Usman and Qureshi, Rizwan and Shah, Abbas and Irfan, Muhammad and Zafar, Anas and Shaikh, Muhammad Bilal and Akhtar, Naveed and Wu, Jia and Mirjalili, Seyedali and others},
  journal={Authorea Preprints},
  year={2023},
  publisher={Authorea}
}

@article{zhao2024revolutionizing,
  title={Revolutionizing Finance with LLMs: An Overview of Applications and Insights},
  author={Zhao, Huaqin and Liu, Zhengliang and Wu, Zihao and Li, Yiwei and Yang, Tianze and Shu, Peng and Xu, Shaochen and Dai, Haixing and Zhao, Lin and Mai, Gengchen and others},
  journal={arXiv preprint arXiv:2401.11641},
  year={2024}
}

@misc{ling2023domain,
      title={Domain Specialization as the Key to Make Large Language Models Disruptive: A Comprehensive Survey}, 
      author={Chen Ling and Xujiang Zhao and Jiaying Lu and Chengyuan Deng and Can Zheng and Junxiang Wang and Tanmoy Chowdhury and Yun Li and Hejie Cui and Xuchao Zhang and Tianjiao Zhao and Amit Panalkar and Wei Cheng and Haoyu Wang and Yanchi Liu and Zhengzhang Chen and Haifeng Chen and Chris White and Quanquan Gu and Jian Pei and Liang Zhao},
      year={2023},
      eprint={2305.18703},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}


@article{hosseini2023exploratory,
  title={An exploratory survey about using ChatGPT in education, healthcare, and research},
  author={Hosseini, Mohammad and Gao, Catherine A and Liebovitz, David M and Carvalho, Alexandre M and Ahmad, Faraz S and Luo, Yuan and MacDonald, Ngan and Holmes, Kristi L and Kho, Abel},
  journal={medRxiv},
  pages={2023--03},
  year={2023},
  publisher={Cold Spring Harbor Laboratory Press}
}

@article{yan2023practical,
  title={Practical and ethical challenges of large language models in education: A systematic literature review},
  author={Yan, Lixiang and Sha, Lele and Zhao, Linxuan and Li, Yuheng and Martinez-Maldonado, Roberto and Chen, Guanliang and Li, Xinyu and Jin, Yueqiao and Ga{\v{s}}evi{\'c}, Dragan},
  journal={arXiv preprint arXiv:2303.13379},
  year={2023}
}


@inproceedings{moore2023empowering,
  title={Empowering education with llms-the next-gen interface and content generation},
  author={Moore, Steven and Tong, Richard and Singh, Anjali and Liu, Zitao and Hu, Xiangen and Lu, Yu and Liang, Joleen and Cao, Chen and Khosravi, Hassan and Denny, Paul and others},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={32--37},
  year={2023},
  organization={Springer}
}

@article{gage1994new,
  title={A new algorithm for data compression},
  author={Gage, Philip},
  journal={C Users Journal},
  volume={12},
  number={2},
  pages={23--38},
  year={1994},
  publisher={McPherson, KS: R \& D Publications, c1987-1994.}
}

@misc{jin2024timellm,
      title={Time-LLM: Time Series Forecasting by Reprogramming Large Language Models}, 
      author={Ming Jin and Shiyu Wang and Lintao Ma and Zhixuan Chu and James Y. Zhang and Xiaoming Shi and Pin-Yu Chen and Yuxuan Liang and Yuan-Fang Li and Shirui Pan and Qingsong Wen},
      year={2024},
      eprint={2310.01728},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

==> backup_introduction.tex <==


\section{Introduction}
\label{sec:intro}


A time series is a sequence of data points, typically recorded at successive equally spaced intervals of time. These data points can represent various measurements, observations, or readings taken over time, such as temperature readings, stock prices, sales figures, or sensor readings. Time series analysis involves studying the patterns, trends, and relationships present in the data to understand its behavior over time. Time series forecasting predicts future
values of a time series $\{y_{t}\}$ based on its past observations. 

Given a historical time series $\{y_{t_1}, y_{t_2}, \dots, y_{t_n}\}$
observed up to time $t_n$, the goal is to predict future values 
$\hat{y}_{t_{n+1}}, \hat{y}_{t_{n+2}}, \hat{y}_{t_{n+m}}$ at time points
$t_{n+1}, t_{n+2}, \dots, t_{n+m}$, where $m$ is the forecasting horizon.  

There are several challenges associated with time series forecasting.
They can for example involve a large number of variables, leading to high-dimensional data sets. Forecasting models need to effectively capture the complex interactions and dependencies among these variables, which can become computationally intensive and challenging. Moreover, variables may exhibit cross-variable dependencies, where the values of one variable depend on the values of other variables at previous time points. Time series data may exhibit complex temporal dynamics, forecasting methods need to account for these temporal dynamics and adapt to changing patterns over time. Time series data sets may suffer from data sparsity or missing values, where certain variables have incomplete or missing observations at specific time points. Handling missing data effectively is crucial for building reliable forecasting models. Furthermore, models can become increasingly complex as the number of variables and the complexity of the relationships among them grow. Balancing model complexity with interpretability is essential for understanding the underlying dynamics and making informed decisions.

Traditional methods for time series forecasting have demonstrated considerable efficacy over the years and continue to maintain relevance and widespread adoption in contemporary practice
\cite{Zeng_Chen_Zhang_Xu_2023}. Broadly, these methods can be categorized into linear and nonlinear models.

Linear methods, see for example \cite{9461796},
\cite{DEGOOIJER2006443} use statistical techniques that assume a linear relationship between the variables involved. These include autoregressive (AR), moving average (MA), autoregressive moving average (ARMA), and autoregressive integrated moving average (ARIMA)~\cite{box2015time} methods. 

AR methods assume that the current value of a time series variable is a linear combination of its past values, with the addition of a white noise term, MA methods
assume that the current value of a time series variable is a linear combination of past white noise terms, with no dependence on past values of the variable itself, ARMA methods combine the characteristics of AR and MA models representing the current value of a time series variable as a linear combination of both its past values and past white noise terms. ARIMA models extend ARMA models by incorporating differencing to make the time series stationary, allowing for the modeling of non-stationary time series data.


Nonlinear methods, see for example \cite{10.1007/11579427_51}, \cite{doi:10.1080/0740817X.2014.999180}
assume a nonlinear relationship between the variables involved and can capture more complex patterns and relationships. Some common nonlinear models in time series forecasting include Threshold Autoregressive (TAR) models, Constant Conditional Correlation (CCC) models, Exponential Smoothing (ES) models, Gaussian Process (GP) models, Kernel Regression (KR) models and Conditional Heteroscedasticity (CH) models. 

TAR models assume different autoregressive relationships 
between variables based on the value of threshold variables,
In CCC models, the correlation matrix is assumed to be constant conditional on past information. 
This means that while the individual variances of each variable may change over time,
the pairwise correlations remain constant. 
ES models are based on the principle of giving exponentially decreasing weights to past observations,
with more recent observations receiving higher weights.
The general idea is to update the forecast at each time step by
combining the observed value at that time with the previous forecast,
adjusting the contribution of past observations using a smoothing parameter.
The smoothing parameter controls the rate at which the weights decrease exponentially.
GP models are nonparametric Bayesian models that 
represent the underlying time series as a distribution over
functions rather than a single deterministic function and
KR models are also nonparametric trying to estimate 
the conditional expectation by weighting the observed data points
according to their proximity to the target points using a kernel function.
The kernel function quantifies the similarity or distance between the target point and each observed data point.
Points closer to the target point are assigned higher weights, indicating greater
influence on the estimated conditional expectation.

In traditional time series analysis, it is often assumed that the variance of the errors or residuals
in a model is constant over time, a property known as homoscedasticity. 
However, in many scenarios, this is not the case and the volatility varies over time.
There may be for example time periods of high volatility and periods of low volatility 
Conditional heteroscedasticity models address this issue by modeling the conditional
variance of the time series, allowing it to vary over time depending on past observations.
These models specify a relationship between the current variance of the series and
its past values or past squared errors.

Machine learning and in particular deep learning has emerged as a transformative approach in the field of time series forecasting, offering new advances in prediction of complex temporal data.
Many different architectures have been used like
recurrent neural networks, convolutional neural networks, transformers and their variants,
see for example \cite{10.1145/3533382}, \cite{doi:10.1089/big.2020.0159},
\cite{Mahmoud2021}, and \cite{DU2020269}.
Unlike traditional statistical
methods, deep learning models can automatically learn hierarchical
representations of the data, enabling learning from the raw
input without the need of preprocessing. 

Pretraining has been a used in deep learning,
to significantly expedite the training process and increase performance \cite{jiang2022transferability}.
In domains such as computer vision and natural language processing,
where vast pretraining datasets exist, pretraining facilitates
the scaling of performance with the availability of data.
However, in the context of time series modeling, access to sizable
pretraining datasets is often limited, hindering the widespread adoption
of pretraining techniques.

In this work, we address this challenge by examining the utility of Large Language Models (LLMs). LLMs are pretrained on vast amounts of text data to learn rich representations of language. These representations capture syntactic, semantic, and contextual information, enabling LLMs to generate coherent and contextually relevant text. By leveraging the prelearned representations of language, LLMs can potentially capture temporal relationships and time series dynamics. We illustrate how pretrained LLMs can be effectively employed in the context of multidimensional time series forecasting as zero-shot learners.

Our contributions are summarized as follows:
\begin{itemize}
    %\item We employ a few-shot technique for LLM-based time series forecasting.
    \item We introduce a dimensional multiplexing technique to combine all dimensions into a single string, passed to an LLM as input.
    \item We employ SAX quantization on the time series to facilitate inference by the model and to significantly reduce the computational cost, making it suitable for use on CPUs.
    \item We present an experimental evaluation against existing traditional, machine learning and LLM-based methods for time series forecasting.
\end{itemize}
